Integrating Chain-of-Thought for Multimodal Alignment: A Study on 3D Vision-Language Learning

Chain-of-Thought (CoT) reasoning has proven effective in natural language tasks but remains underexplored in multimodal alignment. This study investigates its integration into 3D vision-language learning by embedding structured reasoning into alignment training. We introduce the 3D-CoT Benchmark, a dataset with hierarchical CoT annotations covering shape recognition, functional inference, and causal reasoning. Through controlled experiments, we compare CoT-structured and standard textual annotations across large reasoning models (LRMs) and large language models (LLMs). Our evaluation employs a dual-layer framework assessing both intermediate reasoning and final inference quality. Extensive experiments demonstrate that CoT significantly improves 3D semantic grounding, with LRMs leveraging CoT more effectively than LLMs. Furthermore, we highlight that annotation structure influences performance-explicit reasoning markers aid LLMs, while unmarked CoT better aligns with LRM inference patterns. Our analyses suggest that CoT is crucial for enhancing multimodal reasoning, with implications beyond 3D tasks. The dataset will be publicly available at https://huggingface.co/datasets/Battam/3D-CoT

==> sec/3_mathod_refine.tex <==
\section{Method}
\label{sec:method}

We propose a multimodal alignment approach that integrates Chain-of-Thought (CoT) reasoning into 3D vision-language tasks. Specifically, we construct a structured reasoning annotation benchmark (\textit{3D-CoT Benchmark}), design an efficient cross-modal fusion architecture, and employ a two-stage training strategy to achieve deep alignment between 3D structural information and textual reasoning.

\subsection{Method Overview}

As illustrated in Figure~\ref{fig:cot_types}, our approach enhances semantic alignment between 3D vision and language through structured reasoning, facilitating the integration of low-level geometric features with high-level semantic reasoning. Given a 3D point cloud $\mathbf{P}$ and a textual description $\mathbf{T}$, they are encoded into latent space representations $\mathbf{z}_{\mathrm{3D}}$ and $\mathbf{z}_{\mathrm{text}}$, respectively, and mapped into a shared embedding space to establish cross-modal associations. The proposed framework consists of the following key components:

\begin{enumerate}[leftmargin=1.5em]
    \item Construction of the structured reasoning-based \textit{3D-CoT Benchmark} (Sec.~\ref{subsec:benchmark}).
    \item Design of a cross-modal fusion architecture for deep integration of geometric features and chain-of-thought textual reasoning (Sec.~\ref{subsec:architecture}).
    \item A two-stage training strategy to progressively achieve semantic alignment between 3D vision and language (Sec.~\ref{subsec:two_stage_training}).
\end{enumerate}

The following subsections elaborate on each component.

\subsection{3D-CoT Benchmark Construction}
\label{subsec:benchmark}

To provide effective structured reasoning signals, we construct the \textit{3D-CoT Benchmark} based on multiple 3D datasets, including Objaverse~\cite{deitke2023objaverse}, ShapeNet~\cite{chang2015shapenet}, ABO~\cite{collins2022abo}, and 3D-FUTURE~\cite{fu20213d}. The benchmark consists of structured annotations covering:

\begin{itemize}[leftmargin=1.5em]
    \item \textit{Object recognition}: Identifying object categories and fundamental structural attributes.
    \item \textit{Functional inference}: Describing the intended purpose and affordances of objects and their components.
    \item \textit{Causal reasoning}: Explaining how specific structural attributes support or constrain real-world interactions.
\end{itemize}

To investigate the impact of different structured reasoning annotation styles, we generate three distinct formats of textual descriptions:

\begin{itemize}[leftmargin=1.5em]
    \item \textit{Tagged CoT}: Explicitly marked reasoning steps to enhance model recognition of reasoning structures.
    \item \textit{Unmarked CoT}: Multi-step reasoning presented in continuous text, encouraging implicit reasoning without explicit markers.
    \item \textit{No CoT}: Concise descriptions without structured reasoning, serving as a control baseline.
\end{itemize}

Annotations are generated through a two-step process: first, GPT-4o is used to automatically generate initial annotations, followed by human review and refinement on 20\% of the samples to ensure data quality and accuracy.

The benchmark dataset consists of the following components:

\begin{itemize}[leftmargin=1.5em]
    \item \textbf{CoT-CAP3D}: A large-scale multimodal alignment dataset (1.51M samples), with each sample available in both Tagged and Unmarked CoT formats.
    \item \textbf{CoT-CAP3D-SFT}: A subset of 90K samples designed for shape recognition and general functional reasoning.
    \item \textbf{CoT-GApartNet-SFT}: A subset of 54K samples focusing on part-level affordances and fine-grained causal reasoning.
    \item \textbf{Evaluation Sets}: 100 carefully curated test samples per subset, allowing controlled comparisons between different annotation formats and reasoning granularities.
\end{itemize}

\subsection{Cross-modal Fusion Architecture}
\label{subsec:architecture}

To achieve effective alignment between structured textual reasoning and 3D vision features, we design an efficient multimodal fusion architecture consisting of the following components:

\paragraph{3D Feature Extraction}  
We adopt the ReCon++ point cloud encoder~\cite{qi2024shapellm}, which employs farthest point sampling and local feature aggregation to extract both global and local geometric information. The encoder outputs a high-dimensional global embedding vector $\mathbf{e}_{\mathrm{3D}}\in\mathbb{R}^d$ that captures structural details essential for reasoning.

\paragraph{Cross-modal Projection Module}  
A projection network $g_{\mathrm{proj}}(\cdot)$ is designed to map the 3D geometric embedding into a semantically rich, text-compatible space:

\begin{equation}
    \mathbf{z}_{\mathrm{3D}} = g_{\mathrm{proj}}(\mathbf{e}_{\mathrm{3D}}),
\end{equation}

where $\mathbf{z}_{\mathrm{3D}}\in\mathbb{R}^{d'}$. The projection module consists of three MLP-based sub-networks:

\begin{itemize}[leftmargin=1.5em]
    \item A \textbf{local feature projector} to enhance fine-grained geometric details.
    \item A \textbf{global feature projector} to preserve high-level semantics.
    \item An \textbf{absolute position encoding projector} to inject spatial position information.
\end{itemize}

Textual embeddings $\mathbf{z}_{\mathrm{text}}$ are extracted from a pretrained language model, and cross-modal alignment is enforced via a contrastive loss:

\begin{equation}
    \mathcal{L}_{\mathrm{align}} = \text{Contrastive}\left(\mathbf{z}_{\mathrm{3D}}, \mathbf{z}_{\mathrm{text}}\right).
\end{equation}

This multi-projector setup ensures a robust shared embedding space, capturing diverse structural and semantic aspects.

\subsection{Two-Stage Progressive Training}
\label{subsec:two_stage_training}

To progressively align 3D vision and textual reasoning, we propose a two-stage training strategy:

\paragraph{Stage 1: Baseline Cross-modal Alignment}  
The language model remains frozen, and only the projection module is optimized to align 3D features with textual embeddings. This stage utilizes three annotation types: Tagged CoT, Unmarked CoT, and No CoT, enabling the model to acquire fundamental cross-modal mapping capabilities.

\paragraph{Stage 2: Structured Reasoning Integration}  
Selected layers of the language model are unfrozen to facilitate deeper fusion between 3D structural features and textual reasoning. This stage focuses on training with Tagged and Unmarked CoT annotations and examines the impact of explicit versus implicit structured reasoning on cross-modal inference:

\begin{itemize}[leftmargin=1.5em]
    \item \textit{Tagged CoT}: Explicit reasoning step markers guide the model in learning well-defined reasoning structures.
    \item \textit{Unmarked CoT}: Without explicit step markers, the model is encouraged to infer reasoning steps implicitly, promoting more natural integration.
\end{itemize}
